First principles elastic constants and electronic structure of alpha-Pt_2Si and PtSi

We have carried out a first principles study of the elastic properties and electronic structure for two room-temperature stable Pt silicide phases, tetragonal alpha-Pt_2Si and orthorhombic PtSi. We have calculated all of the equilibrium structural parameters for both phases: the a and c lattice constants for alpha-Pt_2Si and the a, b, and c lattice constants and four internal structural parameters for PtSi. These results agree closely with experimental data. We have also calculated the zero-pressure elastic constants, confirming prior results for pure Pt and Si and predicting values for the six (nine) independent, non-zero elastic constants of alpha-Pt_2Si (PtSi). These calculations include a full treatment of all relevant internal displacements induced by the elastic strains, including an explicit determination of the dimensionless internal displacement parameters for the three strains in alpha-Pt_2Si for which they are non-zero. We have analyzed the trends in the calculated elastic constants, both within a given material as well as between the two silicides and the pure Pt and Si phases. The calculated electronic structure confirms that the two silicides are poor metals with a low density of states at the Fermi level, and consequently we expect that the Drude component of the optical absorption will be much smaller than in good metals such as pure Pt. This observation, combined with the topology found in the first principles spin-orbit split band structure, suggests that it may be important to include the interband contribution to the optical absorption, even in the infrared region.

==> prmulticol.tex <==
% Phys-Rev-TeX-files twocolumn

% \narrowtext and \widetext are redefined using the multicol package
% such that we can switch back and forth between narrow and wide
% text. Note that we have to terminate every \narrowtext with \widetext

% Works fine with revtex-3.1

% Roland Winkler

\RequirePackage{multicol}

\newif\ifmynarrow \mynarrowfalse

\parskip 0pt %plus 1pt

\renewcommand{\narrowtext}{%
  \ifmynarrow\hspace*{\fill}\raisebox{-1ex}[0pt][0pt]{%
    \rule{0.3pt}{1ex}%
    \rule[1ex]{20.5pc}{0.3pt}}\fi
  \mynarrowtrue
  \vspace{-1.0ex}%
  \begin{multicols}{2}%
  \par\global\columnwidth20.5pc
  \global\hsize\columnwidth\global\linewidth\columnwidth
  \global\displaywidth\columnwidth}

\renewcommand{\widetext}{%
  \end{multicols}%
  \vspace{-2.5ex}%
  \noindent\raisebox{1ex}[0pt][0pt]{%
    \rule{20.5pc}{0.3pt}%
    \rule{0.3pt}{1ex}}%
  \par\global\columnwidth42.5pc
  \global\hsize\columnwidth\global\linewidth\columnwidth
  \global\displaywidth\columnwidth}

